Neural Graph Collaborative Filtering

Learning vector representations (aka. embeddings) of users and items lies at the core of modern recommender systems. Ranging from early matrix factorization to recently emerged deep learning based methods, existing efforts typically obtain a user's (or an item's) embedding by mapping from pre-existing features that describe the user (or the item), such as ID and attributes. We argue that an inherent drawback of such methods is that, the collaborative signal, which is latent in user-item interactions, is not encoded in the embedding process. As such, the resultant embeddings may not be sufficient to capture the collaborative filtering effect. In this work, we propose to integrate the user-item interactions -- more specifically the bipartite graph structure -- into the embedding process. We develop a new recommendation framework Neural Graph Collaborative Filtering (NGCF), which exploits the user-item graph structure by propagating embeddings on it. This leads to the expressive modeling of high-order connectivity in user-item graph, effectively injecting the collaborative signal into the embedding process in an explicit manner. We conduct extensive experiments on three public benchmarks, demonstrating significant improvements over several state-of-the-art models like HOP-Rec and Collaborative Memory Network. Further analysis verifies the importance of embedding propagation for learning better user and item representations, justifying the rationality and effectiveness of NGCF. Codes are available at https://github.com/xiangwang1223/neural_graph_collaborative_filtering.

==> 5_related.tex <==
\section{Related Work}
According to the manners of modeling the CF effect, especially high-order connectivity, we categorize previous studies related to our work into two fashions: embedding-based and graph-based.

\subsection{Embedding-based Methods}
A line of research~\cite{MF,BPRMF,NCF,WideDeep,DIN,DeepCrossing}, well-known as factorization model, exploits the direct user-item connections by reconstructing historical interactions.
Much effort in both industry and academia has been devoted, revolving two components: embedding and interaction functions.
In particular, embedding function aims to transform users and items to vectorized representations; meanwhile, interaction function estimates a user's preference on an item based on their representations.
In terms of embedding function, matrix factorization (MF)~\cite{MF,BPRMF} presents ID of each user and item as an embedding vector.
Many variants~\cite{VBPR,CKE,CDL} incorporate side information like item content, social relations, and external knowledge to enrich these embeddings.
For instance, collaborative deep learning (CDL)~\cite{CDL} feeds item ID and affiliated texts into the embedding function; collaborative knowledge-based embedding (CKE)~\cite{CKE} combines the representations extracted from the images and knowledge graph with the embedding vector.
Thereafter, the inner product of the user and item embeddings is adopted to calculate their relevance score.
Recent literatures~\cite{NCF,WideDeep,DIN,DeepCrossing,TransRec} focus on exploiting deep learning methods to enhance the interaction function learning, capturing the nonlinear feature interactions or relations between users and items.
For example, neural collaborative filtering (NCF)~\cite{NCF} employs nonlinear neural networks as the interaction function. Wide\&Deep~\cite{WideDeep} contains a deep component, implemented with a neural network, to reveal nonlinear patterns between users and items.
TransRec~\citep{TransRec} leverages the translational principle to capture the user preferences, as well as the sequential
item-item relations.

Despite great success, how the CF effect is captured in these models is opaque, since the collaborative signals are propagated among user- and item-embeddings as the backpropagation of gradients during the optimization process.
Moreover, the neural models are usually trained over the pretrained embeddings of users and items, since the CF effect is hardly captured when learning from scratch.

 

\subsection{Graph-based Methods}
Another line of research~\cite{TrustWalker,BiRank,HOP-rec,DBLP:conf/www/ZhouZYSTZG08,RippleNet,KGAT} exploits higher-order connectivity information between users and items to infer user preferences.
For instance, TrustWalker~\cite{TrustWalker} performs random walks to directly propagate the preference score.
These early methods, however, belong to the regime of label propagation, since none of them encodes connectivity information in the embedding space.

Recently emerged GNNs~\cite{GCN,JumpKG} offers us a chance to perform embedding propagation (or message passing) along the graph structure.
At its core is the neighborhood aggregation, which iteratively aggregates the representations of each node with that of its adjacent nodes as its new representations.
Inspired by the idea, researchers attempt to leverage GNNs to model high-order connectivity in recommender systems~\cite{GC-MC,SpectralCF,RM-GCN}.
For example, RM-GCN~\cite{RM-GCN} performs random walks to generate the neighbors for items, and employs the graph convolutional networks~\cite{GCN} to update the item representations.
SpectralCF~\cite{SpectralCF} considers the connectivity information in the spectral graph.
However, these methods either need the random walk or suffer from the complexity issue, failing to fully explore the higher-order connectivity.


% \section{Related Work}
% According to the manners of modeling the CF effect, we categorize previous studies related to our work into four fashions: neighborhood-based, model-based, hybrid, and graph-based.

% \subsection{Neighborhood-based Methods}
% In the literature of neighborhood-based methods, prior efforts~\cite{CFsurvey,KNN,DBLP:conf/www/DasDGR07} directly implement the CF by estimating similarity between the target item and the historical interactions.
% For example, given a target item, $K$-nearest neighbor (KNN)~\cite{KNN} identifies the similar top $K$ nearest neighbors from the interaction history, and then combines the ratings of these items as the final prediction.
% Due to its simplicity, the neighborhood-based methods are widely used in industry like Amazon~\cite{KNN} and Google News~\cite{DBLP:conf/www/DasDGR07} to generate a candidate list of items.
% However, such methods usually need to estimate user-user or item-item correlations based on the pre-existing features, relying heavily on the choice of the similarity function.



% \subsection{Model-based Methods}
% Prior works~\cite{MF,BPRMF,NCF,WideDeep,DIN,DeepCrossing} parameterize users and items by reconstructing user-item interactions and infer user preferences based on model parameters.
% Much effort in both industry and academia has been devoted, revolving two components: embedding and interaction functions.
% In particular, embedding function aims to transform users and items to vectorized representations; meanwhile, interaction function estimates a user's preference on an item based on their representations.
% In terms of embedding function, matrix factorization (MF)~\cite{MF,BPRMF} presents ID of each user and item as an embedding vector.
% Many variants~\cite{VBPR,CKE,CDL,DBLP:conf/sigir/HuangZDWC18} incorporate side information like item content, social relations, and external knowledge to enrich these embeddings.
% For instance, collaborative deep learning (CDL)~\cite{CDL} feeds item ID and affiliated texts into the embedding function; collaborative knowledge-based embedding (CKE)~\cite{CKE} combines the representations extracted from the images and knowledge graph with the embedding vector.
% Thereafter, the inner product of the user and item embeddings is adopted to calculate their relevance score.
% Recent literatures~\cite{NCF,WideDeep,DIN,DeepCrossing,TransRec} focus on exploiting deep learning methods to enhance the interaction function learning, capturing the nonlinear feature interactions or relations between users and items.
% For example, neural collaborative filtering (NCF)~\cite{NCF} employs nonlinear neural networks as the interaction function. Wide\&Deep~\cite{WideDeep} contains a deep component, implemented with a neural network, to reveal nonlinear patterns between users and items.
% TransRec~\citep{TransRec} leverages the translational principle to capture the user preferences, as well as the sequential
% item-item relations.

% Despite great success, how the CF effect is captured in such models is opaque, since the CF signals are captured as the backpropagation of gradients during the optimization process.
% Moreover, these neural models are usually trained over the pretrained embeddings of users and items, since the CF effect is hardly captured when learning from scratch.

% \subsection{Hybrid Methods}
% Some research efforts~\cite{SVDFeatures,FISM,ACF,DKN,NFM} combine neighborhood-based and model-based CF by introducing the learning of item similarity in the embedding function.
% The basic idea is that the historically interacted items form a user's preference distribution.
% For example, SVD++~\cite{SVDFeatures} aggregates embeddings of the historical items to characterize a user.
% ACF~\cite{ACF} uses the attention mechanism to assign attentive weights to different items to represent a user.
% Factorization Machine (FM)~\cite{FM} and NFM~\cite{NFM} take a user-item pair with her interaction history as generalized features, and integrate all second-order cross features to represent a user's preference.

% Although the CF effect can be captured during the similarity learning process, such methods fail to model the signals carried by the higher-order connectivity between users and items.

% \subsection{Graph-based Methods}
% A line of research~\cite{TrustWalker,BiRank,HOP-rec,DBLP:conf/www/ZhouZYSTZG08,RippleNet} exploits higher-order connectivity information between users and items to infer user preferences.
% For instance, TrustWalker~\cite{TrustWalker} performs random walks to directly propagate the preference score.
% Nevertheless, none of them leverage it in the embedding space.

% More recently, researchers attempt to leverage graph neural networks to model higher-order connectivity in the embedding function~\cite{GC-MC,SpectralCF,RM-GCN}.
% At it core is the message-passing mechanism, where the representation of a node can be propagated to its neighbors.
% For example, RM-GCN~\cite{RM-GCN} performs random walks to generate the neighbors for items, and employs the graph convolutional networks to update the item representations.
% SpectralCF~\cite{SpectralCF} considers the connectivity information in the spectral graph.
% However, these methods either need the random walk or suffer from the complexity issue, failing to fully explore the higher-order connectivity.



